MetricPrompt: Prompting Model as a Relevance Metric for Few-shot Text Classification

Prompting methods have shown impressive performance in a variety of text mining tasks and applications, especially few-shot ones. Despite the promising prospects, the performance of prompting model largely depends on the design of prompt template and verbalizer. In this work, we propose MetricPrompt, which eases verbalizer design difficulty by reformulating few-shot text classification task into text pair relevance estimation task. MetricPrompt adopts prompting model as the relevance metric, further bridging the gap between Pre-trained Language Model's (PLM) pre-training objective and text classification task, making possible PLM's smooth adaption. Taking a training sample and a query one simultaneously, MetricPrompt captures cross-sample relevance information for accurate relevance estimation. We conduct experiments on three widely used text classification datasets across four few-shot settings. Results show that MetricPrompt outperforms manual verbalizer and other automatic verbalizer design methods across all few-shot settings, achieving new state-of-the-art (SOTA) performance.

==> 2_background_short.tex <==

% \section{Preliminaries and Related Work}
% In this section, we review recent works related to the proposed method, and introduce preliminaries revolving prompting models and verbalizer design techniques. 

\section{Preliminaries and Related Work}

\subsection{Prompting methods}
% Traditionally, PLM is adapted to downstream tasks via vanilla fine-tuning. 
% As shown in Fig~\ref{fig:background}, fine-tuning pools PLM's last layer hidden states to form a sentence representation, and makes predictions by feeding the representation to a task-specific classification  head. 
% Fine-tuning is effective given sufficient training data, but its performance degrades significantly under few-shot scenario. 
% The newly initialized task-specific head is prone to over-fitting problem because of the scarcity of supervision signal, and the gap between downstream task formulation and the pre-training objective hinders PLM's smooth adaption. 

Prompting methods are proposed to reformulate downstream tasks to enable PLM's smooth adaption to new tasks. 
% A prompting model's pipeline is illustrated in Fig~\ref{fig:background}.
Denoting $p(\cdot)$ as the prompting function which fills the input text $\mathbf{x}$ into a prompt template, prompting model takes the prompted text and produces output word probability distribution over the vocabulary:
\begin{equation}
\label{eq: background_1}
f_{vocab}(p(\mathbf{x}); \theta) = P(p(\mathbf{x}); \theta), 
\end{equation}
where $P(\cdot; \theta)$ is a PLM parameterized by $\theta$. 
The output word probability $f_{vocab}(\cdot; \theta)$ is then mapped to the final predicted probability distribution over classes with a verbalizer $v(\cdot)$:
\begin{equation}
\label{eq: background_2}
f_{cls}(p(\mathbf{x}); \theta) = v(f_{vocab}(p(\mathbf{x}); \theta)).  
\end{equation}
% Taking news topic classification task as an example, if we want to classify news ``Messi won the World Cup" with a Masked Language Model (MLM), we can prompt it with a template ``\texttt{<text>} The topic of the news is \texttt{[MASK]}". 
% A verbalizer maps the output word at \texttt{[MASK]} position to topic labels.
% For instance, `sports' and `athlete' can be mapped to sports topic, while `diplomacy' and `government' can be aligned to politics topic. 

First proposed by~\citeauthor{radford2019language}, prompting methods have been used in a variety of text mining tasks, such as text classification~\cite{puri2019zero, schick2021eacl, PET, P-tuning}, text generation~\cite{schick2020few, li2021prefix, chen2021evaluating}, named entity recognition~\cite{cui2021template, hou2022inverse}, knowledge probing~\cite{petroni2019language, talmor2020olmpics}, etc. 
Prompting model alleviates the over-fitting problem under few-shot scenario significantly~\cite{brown2020language, PET, tam2021improving}. 
However, prompting model's performance relies largely on the selection of prompt template and verbalizer~\cite{liu2021pre}. 
Although a number of works focus on the design of prompt~\cite{gao2020making, shin2020autoprompt, li2021prefix, P-tuning}, less are proposed to ease verbalizer design difficulty. 
Verbalizer maps prompting model's output words to classification results directly, and therefore influences prompting model's performance significantly~\cite{gao2020making}.
In this work, we seek to free human labor from verbalizer design with less performance loss.


\subsection{Verbalizer Design Methods}
% \begin{figure*}[t]
% \centering
% \begin{tikzpicture}
% \draw (0,0 ) node[inner sep=0] {\includegraphics[width=2\columnwidth, trim={0cm 1cm 2cm 0cm}, clip]{./figs/MetricPrompt.pdf}};
% \end{tikzpicture}
% \caption{
% A demonstration of Metricprompt's data construction and functioning procedure. 
% }\label{fig:method}
% \end{figure*}

Current verbalizer design methods can be classified into manual verbalizer design, discrete verbalizer design and soft verbalizer design. 
A carefully hand-crafted verbalizer can achieve highly competitive performance in various NLP tasks~\cite{PET, schick2021eacl}. 
However, designing such a well-performing verbalizer relies heavily on human's accurate understanding of the target task and requires heavy trial-and-error work. 
Discrete verbalizer design methods frees human labor from verbalizer design by generating verbalizer with larger language models~\cite{gao2020making}, optimizing randomly constructed verbalizer~\cite{shin2020autoprompt,schick2021eacl} or selecting words to maximize the likelihood of the training data~\cite{schick2020coling}. 
% LM-BFF~\cite{gao2020making} generates proper answer words with large PLMs such as T5~\cite{raffel2019exploring}.
% AutoPrompt~\cite{shin2020autoprompt} and AVS~\cite{schick2021eacl} initialize a verbalizer and optimize it to meet a predefined criteria iteratively. 
% PETAL~\cite{schick2020coling} searches for answer words that maximize the likelihood of the training data.
However, these methods' performance lags far behind carefully hand-crafted verbalizers~\cite{cui2022prototypical}. 
To achieve better performance, soft verbalizer design methods expand verbalizer design space and represent each label with a continuous embedding~\cite{hambardzumyan2021warp, zhang2021differentiable, cui2022prototypical}. 
Nevertheless, task-specific label embeddings are prone to over-fitting problem, and these methods' task formulations are distinct from PLM's pre-training objective. 
% Expanding the possibilities of verbalizer design space, these methods achieve better results than discrete verbalizer design algorithms~\cite{hambardzumyan2021warp, zhang2021differentiable, cui2022prototypical}. 
% However, task-specific label embeddings are prone to over-fitting problem, and these methods functions in a way distinct from PLM' pre-training objective. 

In this work, we ease task-specific verbalizer design difficulty by reformulating text classification task into text pair relevance estimation task. 
% The proposed method introduces no task-specific parameter and operates with only output word probabilities, making 
In this way, no additional task-specific parameter is introduced, and the over-fitting problem is alleviated. 
Adopting prompting model as the relevance metric and operating with only output word probabilities, PLM can adapt to new tasks more smoothly.
A recent work also views text classification task as natural language inference problem~\cite{plaza2022natural}, but it focuses on zero-shot scenario and hand-craft each label's description.
In comparison, our method tackle few-shot text classification tasks instead of zero-shot ones, and does not require human labor in task-specific verbalizer design. 



% Prompting methods are proposed to better utilize Pre-trained Language Models' (PLM) general knowledge in downstream NLP tasks by aligning them to PLMs'  pre-training objectives. 
% Prompting method insert sample news text into prompt template to form prompted text. 
% Taking news topic classification task as an example, if want to classify news ``Messi won the World Cup" with a Masked Language Model (MLM), we can insert it into a prompt template ``\texttt{<text>} The topic of the news is \texttt{[MASK]}". 
% In this way, news topic classification task is reformulated as an MLM problem.
% We can obtain the classification result by mapping the output word at \texttt{[MASK]} position to topic labels. 
% Label mapping is conducted with a \textit{verbalizer}, which computes each label's probability by aggregating its corresponding answer words output probability. 
% % Verbalizer directly maps PLMs' output words to corresponding labels, and therefore influence prompting models' performance greatly. 

% Although achieving promising results a a wide variety of NLP tasks, prompt methods are very susceptible to sub-optimal verbalizer design~\cite{gao2020making}.
% However, designing a proper verbalizer requires deep understanding of both downstream NLP task and PLM's inner mechanism. 
% In practice, this procedure can be extremely resource-consuming. 
% As a result, many researchers seek to automate the verbalizer design process and achieve better results. 
% Automatic verbalizer design methods can be classified in 2 genres: discrete verbalizer design and soft verbalizer design~\cite{liu2021pre}. 
% Discrete verbalizer design methods, such as LM-BFF~\cite{gao2020making} and AutoPrompt~\cite{shin2020autoprompt}, search each label's corresponding answer words with large PLMs, gradient-based algorithms, etc. 
% These methods reduce human labor required by verbalizer design significantly, but their performance lags far behind carefully hand-crafted ones~\cite{cui2022prototypical}. 
% Soft verbalizer design methods are proposed to search for proper verbalizer parameters in an infinite continuous space. Expanding the possibilities of verbalizer design space, these methods achieves better results than discrete verbalizer design algorithms~\cite{hambardzumyan2021warp, cui2022prototypical}. 

% Despite the promising prospects of soft verbalizer, current methods' performance are still far from satisfactory. 
% The first reason is that current soft verbalizer methods' optimization and inference formulation are distinct from PLM's pre-training objective. 
% WARP~\cite{hambardzumyan2021warp} trains each label's soft embedding from scratch on few labeled samples of the downstream task, while ProtoVerb~\cite{cui2022prototypical} takes prompting model as a feature extractor and aggregates each training sample's representation at \texttt{[MASK]} position to form corresponding label's prototypical embedding. 
% Both methods force PLM to adapt to a distinct task formulation from its pre-training objective, and therefore hinder smooth adaption to downstream tasks. 
% What's worse, both WARP and ProtoVerb compute each label and query sample's representation respectively. 
% As a result, the model cannot analyze cross-sample relevance information between training and query samples to aid classification.











==> 3_methods_short.tex <==

\section{Methods}
% Since previous soft verbalizer design methods formulate downstream tasks in a distinct way from PLM's pre-training objective, we introduce MetricPrompt, which further bridges the gap between 
% In this section, we introduce MetricPrompt, which frees human labor from task-specific verbalizer design by rendering prompting model as a metric to estimate the relevance between training and query samples, and making classification predictions with the estimations.
In this section, we introduce the data construction, optimization and inference procedure of MetricPrompt in detail. 

\begin{figure*}[t]
\centering
\begin{tikzpicture}
\draw (0,0 ) node[inner sep=0] {\includegraphics[width=2\columnwidth, trim={0cm 1cm 2cm 0cm}, clip]{./figs/MetricPrompt.pdf}};
\end{tikzpicture}
\caption{
Metricprompt's data construction, training and inference procedure. 
Original data is paired to form positive and negative samples, and the prompting model is optimized to map these samples to corresponding words.  
A query sample is paired with each training sample, and the optimized prompting model is used as a metric to estimate relevance scores, which are pooled to produce final classification results.
}\label{fig:method_1}
\end{figure*}


\subsection{Data construction}
Given a few-shot text classification dataset $\mathcal{D}$, we denote training data with $\mathcal{D}_{t}$ and query samples with $\mathcal{D}_{q}$. 
A sample is formulated as $d=(\mathbf{x}_d, \mathbf{y}_d)$, where $\mathbf{x}_d$ stands for sample text and $\mathbf{y}_d$ represents its label. 
% Since MetricPrompt takes as input a pair of sample text, we construct training data as follows:
We construct training data as follows:
\begin{equation}
\label{eq: data_construction}
\begin{split}
&\mathcal{D}_{t}^{M} = \bigcup_{(d_i, d_j) \in \mathcal{D}_{t} \times \mathcal{D}_{t}} \{ (p(\mathbf{x}_{d_i}, \mathbf{x}_{d_j}), \mathbf{y}_{ij}) \}, \\
&\mathcal{D}_{q}^{M} = \bigcup_{(d_i, d_j) \in \mathcal{D}_{q} \times \mathcal{D}_{t}} \{ (p(\mathbf{x}_{d_i}, \mathbf{x}_{d_j}), \mathbf{y}_{ij}) \},
\end{split}
\end{equation}
where $p(\cdot, \cdot)$ is MetricPrompt's prompting function. 
It takes two pieces of sample text and produces a filled prompt template. 
% We use ``$\mathbf{x}_{d_i}$ \texttt{[SEP]} A news of \texttt{[MASK]} topic: $\mathbf{x}_{d_j}$" as the prompt template. 
$\mathbf{y}_{ij}=\mathbb{I}(\mathbf{y}_{d_i}=\mathbf{y}_{d_j})$ indicates whether the pair of text are of the same class.

% Similarly, we build query data for MetricPrompt as follows:
% \begin{equation}
% \label{eq: data_construction_query}
% \mathcal{D}_{q}^{M} = \bigcup_{(d_i, d_j) \in \mathcal{D}_{q} \times \mathcal{D}_{t}} \{ (p(\mathbf{x}_{d_i}, \mathbf{x}_{d_j}), \mathbf{y}_{ij}) \}.
% \end{equation}

The overall data construction process is illustrated in Fig~\ref{fig:method_1}.
We reorganize the original classification problem to be a relevance estimation task, requiring no label's semantic representation or human labor in task-specific verbalizer design.
% We reorganize single samples of a given few-shot text classification task into paired samples, and the original multi-class classification problem is rendered as a relevance estimation task. 
% No label's semantic representation is involved in this data construction procedure, and therefore MetricPrompt requires no human labor in task-specific verbalizer design.


\subsection{Optimization}

% \begin{figure*}[t]
% \centering
% \begin{tikzpicture}
% \draw (0,0 ) node[inner sep=0] {\includegraphics[width=2\columnwidth, trim={0cm 1cm 2cm 9cm}, clip]{./figs/MetricPrompt.pdf}};
% \end{tikzpicture}
% \caption{
% The inference procedure of MetricPrompt. 
% A query sample is paired with each training sample, and the relevance scores are pooled to produce final classification probabilities.
% }\label{fig:method_2}
% \end{figure*}

MetricPrompt adopts a generalized (M)LM task for optimization, which is consistent with PLM's pre-training objective. 

% Let $P(\cdot;\theta)$ be an MLM model parameterized by $\theta$ and $f_{vocab}(\cdot;\theta)$ be its output word probability over the vocabulary.
We define the optimization objective of MetricPrompt as follows:
\begin{equation}
\label{eq: optimization}
\small
\begin{split}
\hat{\theta} 
&=\mathop{\arg\min}\limits_{\theta} \sum_{d^M \in \mathcal{D}_{t}^{M}} \mathcal{L}(f_{vocab}(\mathbf{x}_{d^M};\theta), \mathbf{y}_{d^M}) \\
&=\mathop{\arg\min}\limits_{\theta} \sum_{d^M \in \mathcal{D}_{t}^{M}} \mathcal{L}_{CE}(f_{cls}(\mathbf{x}_{d^M};\theta)), \phi(\mathbf{y}_{d^M})), 
\end{split}
\end{equation}
where $\phi(\cdot)$ is the probability distribution over label categories. 
The corresponding position of the sample label is set as 1 while others are set to be 0. 
Output word probability $f_{vocab}(\mathbf{x}_{d^M}; \theta)$ is mapped to a binomial distribution $f_{cls}(\mathbf{x}_{d^M}; \theta)$ with a predefined task-general meta verbalizer $v(\cdot)$. 
We task this meta verbalizer to aggregate logits at $\texttt{\{relevant}, \texttt{similar}, \texttt{consistent\}}$ to be the predicted logit of label 1, while logits at $\texttt{\{irrelevant}, \texttt{inconsistent}, \texttt{different\}}$ are aggregated to be the logit of label 0.\footnote{Note that this meta verbalizer can be used in all few-shot text classification tasks, so MetricPrompt requires no extra human labor in task-specific verbalizer design.}
$\mathcal{L}$ is the loss function of MetricPrompt, which is defined as the cross-entropy loss between the probability distributions produced by the meta verbalizer $v(\cdot)$ and the ground truth distribution $\phi(\mathbf{y}_{d^M})$. 

MetricPrompt formulates few-shot text classification task's optimization objective to be a generalized (M)LM task which only involves output word probabilities. 
% which is the minimization of cross-entropy loss between predicted word probability at \texttt{[MASK]} position and the ground truth one-hot distribution. 
% The optimized prompting model can be used as a metric to estimate the relevance between two sample text. 

% adapt epochs?

\subsection{Inference}
After optimization, the prompting model serves as a relevance metric during inference. 
As illustrated in Fig~\ref{fig:method_1}, we take an original query sample $d_q$ colored in black and pair it with all training samples colored differently to form inference samples.
% its paired training samples in other colors to illustrate MetricPrompt's inference process. 
Given an original training sample $d_i$, MetricPrompt computes its relevance score $s_{d_i}$ with $d_q$ as follows:
\begin{equation}
\label{eq: inference_1}
s_{d_i} = \Delta(f_{cls}(p(\mathbf{x}_{d_q}, \mathbf{x}_{d_i}); \hat{\theta})), 
\end{equation}
where $\Delta(\cdot)$ computes the difference between the binomial distribution's probability at 1 and 0. 
We denote $l$ as a label of the few-shot text classification task. 
Let $\mathcal{D}_{l}=\{d_i | d_i \in \mathcal{D}_{t}, \mathbf{y}_{d_i}=l_i\}$, MetricPrompt calculates $l$'s classification score $s_{l}$ by pooling its corresponding samples' relevance with $d_q$:
\begin{equation}
\label{eq: inference_2}
s_{l} 
= \sum_{d_i \in \mathcal{D}_{l}} s_{d_i} / |\mathcal{D}_{l}|. 
\end{equation}
Finally, MetricPrompt selects label $\hat{l}$ with the highest relevance score as the classification result:
\begin{equation}
\label{eq: inference_3}
\hat{l} 
= \mathop{\arg\max}\limits_{l} s_l. 
\end{equation}

We present MetricPrompt with sum pooling in Equation~\ref{eq: inference_2}.
This pooling function can also be replaced by max pooling and K-Nearest-Neighborhood (KNN)~\cite{cover1967nearest} pooling. 
Max pooling classifies query sample $d_q$ into its most relevant training sample's class by replacing Equation~\ref{eq: inference_2} with:
\begin{equation}
\label{eq: inference_4}
s_{l} 
= \max_{d_i \in \mathcal{D}_{l}} s_{d_i}. 
\end{equation}
For KNN pooling, we denote $\mathcal{D}_{topk}$ as $k$ training samples most relevant to $d_q$ and reformulate Equation~\ref{eq: inference_2} as:
\begin{equation}
\label{eq: inference_5}
s_{l} 
= |\{d_i | d_i \in \mathcal{D}_{topk}, \mathbf{y}_{d_i}=l_i\}|. 
\end{equation}
We set $k$ as half the size of training set. 
When several labels appear in $\mathcal{D}_{topk}$ for the same number of times, the query sample is classified to the label of its most relevant training sample. 
% we select the sample obtaining the highest relevance score from these labels' corresponding samples, and classify $d_q$ to its class.
% we select the training sample of the highest relevance score with $d_q$ and classify $d_q$ to its class.

MetricPrompt renders prompting model as a relevance metric, and classifies query samples according to their relevance with training samples of the few-shot task. 
Taking paired text as input, MetricPrompt uses cross-sample information to aid relevance estimation accuracy. 
% Prompting model takes two pieces of sample text at once. 
% Thus, MetricPrompt is able to use cross-sample information to estimate relevance and make predictions accurately. 


\subsection{More Efficient Inference}
% MetricPrompt pairs each query sample with all training samples, leading to relatively high inference cost. 
To improve the efficiency of MetricPrompt, we propose to use pivot samples to reduce inference time complexity. 
We use the optimized prompting model to select representative training samples. 
For a training sample $d_i$ labeled with $l$, its representativeness $r_{d_i}$ as follows:
\begin{equation}
\small
    r_{d_i} 
    = \frac{\sum_{d_j \in \mathcal{D}_l}{s_{d_j}}}{|\{d_j|d_j \in \mathcal{D}_l\}|} - \frac{\sum_{d_k \in \mathcal{D}_t-\mathcal{D}_l}{s_{d_k}}}{|\{d_k|d_k \in \mathcal{D}_t-\mathcal{D}_l\}|}. 
\end{equation}
$s_{d_j}$ represents the relevance score between samples $d_j$ and $d_i$. 
Based on this representativeness metric, we select top $p$ representative samples for each label.
These samples are marked as pivot samples.
% and participate in the inference process. 
During inference, query samples are only paired with these pivot samples to make classification prediction.

Pivot samples reduce the time complexity of MetricPrompt's inference process significantly. 
Assume a few-shot text classification task with $n$ labels and $k$ samples per label.
The introduction of pivot samples reduce the number of each query sample's text pairs for relevance estimation from $n*k$ to $n*p$.
Accordingly, $O(n*k)$ inference time complexity is reduced to $O(n*p)$.
Since $p$ is a pre-defined constant, the improved inference time complexity is $O(n)$, which is equivalent with vanilla prompting method where the input text representation is dot multiplied with each label word's embedding. 
We set the number of pivot samples per label $p$ to 2 in the experiments. 

% Assume a few-shot text classification task with $n$ labels and $k$ samples per label.
% Without introducing pivot samples, MetricPrompt computes relevance scores for $n*k$ text pairs, resulting into $O(n*k)$ inference time complexity. 
% In contrast, prompting methods with human-designed or automatically designed verbalizer calculate the dot product similarity between the feature representations of test samples and feature representation of each label, which is covered with $O(n)$ time complexity. 
% When pivot samples are used, MetricPrompt only needs to estimate the relevance for $n*p$ text pairs, reducing the time complexity to $O(p*n)$, where $p$ is a pre-defined constant. 
% As a result, pivot samples accelerates MetricPrompt's inference process from $O(n*k)$ time complexity to $O(n)$. 
% We set the number of pivot samples per label $p$ to 2 in the experiments.































==> 4_experiments_short.tex <==

\section{Experiments}
% We conduct extensive experiments with MetricPrompt and previous SOTA verbalizer design methods to show MetricPrompt's effectiveness. 
In this section, we first introduce the datasets used in our experiments. 
Then we describe our experiment settings and implementation details. 
Finally, we present experiment results and analyze MetricPrompt's performance.


\subsection{Datasets}
We conduct experiments with three widely used text classification tasks, which contain numerous classes and hence require extensive resources to build a proper manual verbalizer. 
We adopt AG’s News, Yahoo Answers topics~\cite{Zhang2015CharacterlevelCN} and DBPedia~\cite{lehmann2015dbpedia} as our text classification tasks.
The statistics of the datasets are given in Table ~\ref{tbl: datasets_statistics}.

\begin{table}[t]
\small
\begin{tabular}{c c c c}
\toprule
Dataset & \# Class & \# Test & Avg len
\\
\midrule
AG’s News & 4 & 7,600 & 52 \\
DBPedia & 14 & 70,000 & 68 \\
Yahoo & 10 & 60,000 & 130 \\
\bottomrule
\end{tabular}
\centering
\caption{
Statistics of the three text classification datasets used in our experiments. 
}\label{tbl: datasets_statistics}
\end{table}

Since the average text length of the three datasets is short, we truncate all sample text to 120 tokens for better efficiency with little semantic meaning loss.


\subsection{Few-shot experiment settings}
We conduct experiments under 2, 4, 8 and 16-shot settings, where corresponding number of training samples are sampled from each dataset's training set randomly.
% Models' performance are observed to fluctuate largely when the training set is sampled with different random seeds.  
To improve the reliability of evaluation results, we sample 10 training sets for each dataset and few-shot setting and compute the average performance on these training sets. 
% All experiment results are reported as the average value of the model's performance on the 10 training sets. 


\subsection{Implementation Details}
We implement MetricPrompt with PyTorch~\cite{paszke2019pytorch} and Huggingface~\cite{wolf2020transformers} framework, and baselines are implemented with OpenPrompt toolkit~\cite{ding2021openprompt}.
We introduce Kernl to accelerate the inference procedure.\footnote{\href{https://github.com/ELS-RD/kernl}{https://github.com/ELS-RD/kernl}}

We adopt BERT-base-uncased~\cite{devlin2019bert} as the backbone model for both MetricPrompt and all baseline models for fair comparison. 
Model parameters are optimized with AdamW optimizer~\cite{AdamW}, 1e-5 learning rate and 16 batch size.
% We train MetricPrompt for 120 epochs with batch size set as 16 for AG's News dataset 2-shot setting. 
We set total training steps proportionally to the size of training set, and the number of training epochs is given in Table~\ref{tbl: epochs}.
% To realize such a training strategy, the epoch number is decreased proportionally to shot number, because the quantity of trainning samples increases proportionally to its square. 
% The size of training set varies across datasets and shot numbers, and the specific number of training epochs is given in Table~\ref{tbl: epochs}.
% Since the number of class varies across datasets, we also modify the number of training epochs based on the size of their training data, and the specific epoch number is given in Table~\ref{tbl: epochs}.


\subsection{Baselines}
We select several representative verbalizer design methods for comparison.
Among the listed baselines, only manual verbalizer requires human effort in task-specific verbalizer design. 

\textbf{Manual Verbalizer} (ManualVerb) uses hand-crafted verbalizer to map PLM's output word to classification labels. We use the verbalizer provided by OpenPrompt~\cite{ding2021openprompt} in our experiments. 

\textbf{Automatic Verbalize Search} (AVS)~\cite{schick2021eacl} is a search-based verbalizer design method. It initializes the verbalizer with random words, and improves answer words iteratively. 
% Words which the PLM considers to represent the given samples more suitably are selected as replacing words in each iteration. 

\textbf{Soft Verbalizer} (SoftVerb)~\cite{hambardzumyan2021warp} represents each label with a trainable embedding. 
In the original work WARP, the prompt template is also represented as trainable embeddings.
In this work, however, we follow \citeauthor{cui2022prototypical} to use manual template for fair comparison.

\textbf{Prototypical Verbalizer} (ProtoVerb)~\cite{cui2022prototypical} also represents classification labels as soft embeddings but adopts prototypical contrastive learning loss~\cite{liprototypical} instead of vanilla cross-entropy loss to optimize model parameters. 
% \textbf{Prototypical Verbalizer} (ProtoVerb)~\cite{cui2022prototypical} renders prompting model as a feature extractor, which represents sample text with the last layer's hidden states at \texttt{[MASK]} position. 
% The model is optimized with contrastive loss and labels are represented as aggregated prototypes of their corresponding samples. 

We refer to Appendix~\ref{appendix: A} for the specific prompt templates and verbalizers used in our experiments. 

\begin{table}[t]
\small
\begin{tabular}{c c c c c}
\toprule
Dataset & 2-shot & 4-shot & 8-shot & 16-shot
\\
\midrule
AG’s News & 120 & 60 & 30 & 15 \\
DBPedia & 32 & 16 & 8 & 4 \\
Yahoo & 36 & 18 & 9 & 5 \\
\bottomrule
\end{tabular}
\centering
\caption{
The number of training epochs for given datasets and few-shot settings. 
}\label{tbl: epochs}
\end{table}


\subsection{Main Results}
\label{sec: 4_5}

\begin{table*}[t]
% \small
% \resizebox{\textwidth}{15mm}{
\begin{tabular}{l cc cc cc cc}
\toprule
\multicolumn{1}{c}{Method} &
\multicolumn{2}{c}{AG's News} &
\multicolumn{2}{c}{DBPedia} &
\multicolumn{2}{c}{Yahoo} &
\multicolumn{2}{c}{Average}
\\
\cmidrule(lr{0.5em}){2-3}\cmidrule(lr{0.5em}){4-5}\cmidrule(lr{0.5em}){6-7}\cmidrule(lr{0.5em}){8-9} 
& 2-shot & 4-shot & 2-shot & 4-shot & 2-shot & 4-shot & 2-shot & 4-shot 
\\
\midrule
\textsc{ManualVerb}       & $\textit{45.87}$ & $\textit{76.22}$ & $\textit{69.81}$ &  $\textit{84.15}$ & $\textit{34.82}$ &  $\textit{55.56}$ & $\textit{50.17}$ &  $\textit{71.98}$\\
\textsc{AVS}~\citeyearpar{schick2021eacl}        & $44.93$ & $57.49$ & $32.22$ &  $53.55$ & $21.88$ &  $28.44$ & $33.01$ &  $46.49$\\
\textsc{SoftVerb}~\citeyearpar{hambardzumyan2021warp}        & $48.86$ & $61.15$ & $53.98$ & $76.19$ & $22.63$ &  $33.43$ & $41.82$ & $56.92$\\
\textsc{ProtoVerb}~\citeyearpar{cui2022prototypical}        & $58.38$ & $65.04$ & $60.89$ & $74.49$ & $28.80$ &  $43.01$ & $49.36$ & $60.85$\\
\midrule
\textsc{$\text{MetricPrompt}_{\text{knn}}$}     & $62.69$ & $73.17$ & $66.27$ & $86.06$ & $26.02$ &  $50.90$ & $51.66$ &  $70.04$\\
\textsc{$\text{MetricPrompt}_{\text{max}}$}     & $65.64$ & $76.12$ & $\bm{71.28}$ & $\bm{88.44}$ & $\bm{28.85}$ &  $52.99$ & $\bm{55.26}$ &  $72.52$\\
\textsc{$\text{MetricPrompt}_{\text{mean}}$}       & $\bm{65.77}$ & $\bm{76.33}$ & $71.20$ & $\bm{88.44}$ & $28.76$ &  $\bm{53.54}$ & $55.24$ &  $\bm{72.77}$ \\
\textsc{$\text{MetricPrompt}_{\text{pivot}}$}       & $65.76$ & $74.53$ & $71.20$ & $86.12$ & $28.76$ &  $51.32$ & $55.24$ &  $70.66$ \\
\bottomrule
\end{tabular}
% }
\centering
\caption{
Experiment results in terms of accuracy under 2-shot and 4-shot settings. Italic score means human labor is involved in task-specific verbalizer design, and bold number indicates the best result among methods requiring no human labor. 
}
\label{tbl: main_24}
% \vspace{-5mm}
\vspace*{-3mm}
\end{table*}

\begin{table*}[t]
% \small
% \resizebox{\textwidth}{15mm}{
\begin{tabular}{l cc cc cc cc}
\toprule
\multicolumn{1}{c}{Method} &
\multicolumn{2}{c}{AG's News} &
\multicolumn{2}{c}{DBPedia} &
\multicolumn{2}{c}{Yahoo} &
\multicolumn{2}{c}{Average}
\\ 
\cmidrule(lr{0.5em}){2-3}\cmidrule(lr{0.5em}){4-5}\cmidrule(lr{0.5em}){6-7}\cmidrule(lr{0.5em}){8-9} 
& 8-shot & 16-shot & 8-shot & 16-shot & 8-shot & 16-shot & 8-shot & 16-shot 
\\
\midrule
\textsc{ManualVerb}       & $\textit{78.94}$ & $\textit{83.66}$ & $\textit{94.24}$ & $\textit{97.27}$ & $\textit{58.30}$ &  $\textit{62.42}$ & $\textit{77.16}$ & $\textit{81.12}$\\
\textsc{AVS}~\citeyearpar{schick2021eacl}      & $71.37$ & $77.81$ & $75.91$ & $85.36$ & $46.53$ & $57.68$ & $64.60$ &  $73.62$\\
\textsc{SoftVerb}~\citeyearpar{hambardzumyan2021warp}       & $73.28$ & $80.61$ & $90.34$ & $96.93$ & $45.01$ &  $59.09$ & $69.54$ &  $78.88$\\
\textsc{ProtoVerb}~\citeyearpar{cui2022prototypical}       & $75.57$ & $80.31$ & $87.45$ &  $\bm{97.16}$ & $52.87$ &  $61.57$ & $71.96$ &  $79.68$\\
\midrule
\textsc{$\text{MetricPrompt}_{\text{knn}}$}     & $80.64$ & $84.43$ & $94.25$ & $96.55$ & $58.09$ &  $62.05$ & $77.66$ & $81.01$\\
\textsc{$\text{MetricPrompt}_{\text{max}}$}     & $81.03$ & $84.27$ & $94.28$ & $96.55$ & $59.68$ &  $62.66$ & $78.33$ & $81.16$\\
\textsc{$\text{MetricPrompt}_{\text{mean}}$}       &  $\bm{82.04}$ & $\bm{84.69}$ & $\bm{94.57}$ & $96.59$ & $\bm{59.68}$ & $\bm{62.45}$ & $\bm{78.76}$ & $\bm{81.24}$\\
\textsc{$\text{MetricPrompt}_{\text{pivot}}$}       & $81.19$ & $84.15$ & $94.13$ & $96.22$ & $58.63$ &  $61.78$ & $77.98$ &  $80.72$ \\
\bottomrule
\end{tabular}
% }
\centering
\caption{
Experiment results in terms of accuracy under 8-shot and 16-shot settings. Italic score means human labor is involved in task-specific verbalizer design, and bold number indicates the best result among methods requiring no human labor. 
}
\label{tbl: main_816}
% \vspace{-5mm}
\vspace*{-3mm}
\end{table*}

% \begin{table*}[t]
% % \small
% \resizebox{\textwidth}{15mm}{
% \begin{tabular}{l cccc cccc cccc cccc}
% \toprule
% \multicolumn{1}{c}{Method} &
% \multicolumn{4}{c}{AG's News} &
% \multicolumn{4}{c}{DBPedia} &
% \multicolumn{4}{c}{Yahoo} &
% \multicolumn{4}{c}{Average}
% \\
% \cmidrule(lr{0.5em}){2-5}\cmidrule(lr{0.5em}){6-9}\cmidrule(lr{0.5em}){10-13}\cmidrule(lr{0.5em}){14-17} 
% & 2-shot & 4-shot & 8-shot & 16-shot & 2-shot & 4-shot & 8-shot & 16-shot & 2-shot & 4-shot & 8-shot & 16-shot & 2-shot & 4-shot & 8-shot & 16-shot 
% \\
% \midrule
% \textsc{ManualVerb}       & $45.87$ &  $76.22$ & $78.94$ & $83.66$ & $69.81$ &  $84.15$ & $94.24$ &  $97.27$ & $34.82$ &  $55.56$ & $58.30$ &  $62.42$ &  $-$ &  $-$ & $-$ &  $-$\\
% \textsc{AVS}       & $44.93$ & $57.49$ &  $71.37$ & $77.81$ & $-$ &  $-$ & $-$ & $-$ & $21.88$ &  $28.44$ & $46.53$ &  $-$ &  $-$ &  $-$ & $-$ &  $-$\\
% \textsc{SoftVerb}       & $48.86$ & $61.15$ &  $73.28$ & $80.61$ & $53.98$ &  $76.19$ & $90.34$ &  $96.93$ & $22.63$ &  $33.43$ & $45.01$ &  $59.09$ &  $-$ &  $-$ & $-$ &  $-$\\
% \textsc{ProtoVerb}       & $58.38$ & $65.04$ &  $75.57$ & $80.31$ & $60.89$ &  $74.49$ & $87.45$ &  $97.16$ & $28.80$ &  $43.01$ & $52.87$ &  $61.57$ &  $-$ &  $-$ & $-$ &  $-$\\
% \midrule
% \textsc{MetricPrompt}       & $65.77$ & $76.33$ &  $82.04$ & $84.69$ & $71.20$ &  $88.44$ & $94.57$ &  $96.59$ & $28.76$ &  $53.54$ & $59.68$ &  $62.45$ &  $-$ &  $-$ & $-$ &  $-$\\
% \bottomrule
% \end{tabular}
% }
% \centering
% \caption{}
% \label{tbl:main}
% % \vspace{-5mm}
% \vspace*{-3mm}
% \end{table*}


We conduct experiments on three text classification datasets with different text styles under four few-shot settings. 
Experiment results for 2 and 4-shot settings are listed in Table~\ref{tbl: main_24}, while 8 and 16-shot's experiment results are shown in Table~\ref{tbl: main_816}. 
% MetricPrompt outperforms previous SOTA automatic verbalizer design method ProtoVerb by a large margin, improving 2-shot accuracy by $5.88$ ($11.91\%\uparrow$), 4-shot accuracy by $11.92$ ($19.59\%\uparrow$), 8-shot accuracy by $6.80$ ($9.45\%\uparrow$) and 16-shot accuracy by $1.56$ ($1.96\%\uparrow$). 
MetricPrompt outperforms previous SOTA baseline ProtoVerb across all few-shot settings, even surpassing ManualVerb under all without any human labor involved in task-specific verbalizer design. 

\begin{table*}[t]
% \small
\resizebox{\textwidth}{!}{
\begin{tabular}{l ccc l ccc l ccc}
\toprule
\multicolumn{1}{c}{Method} &
\multicolumn{3}{c}{AG's News} &
\multicolumn{1}{c}{Method} &
\multicolumn{3}{c}{DBPedia} &
\multicolumn{1}{c}{Method} &
\multicolumn{3}{c}{Yahoo}
\\
\cmidrule(lr{0.5em}){2-4}\cmidrule(lr{0.5em}){6-8}\cmidrule(lr{0.5em}){10-12}
& 1-shot & 2-shot & 4-shot & & 1-shot & 2-shot & 4-shot & & 1-shot & 2-shot & 4-shot
\\
\midrule
\textsc{ProtoVerb}     & $46.79$ & $58.38$ & $65.04$ & \textsc{ProtoVerb} & $45.86$ & $60.89$ &  $74.49$ & \textsc{ProtoVerb} & $21.60$ & $28.80$ & $43.01$ \\
\quad\textsc{+DBPedia}     & $57.43$ & $65.72$ & $71.27$ & \quad\textsc{+AG's News} & $49.00$ & $63.29$ &  $75.56$ & \quad\textsc{+AG's News} & $28.93$ & $39.15$ & $49.96$ \\
\quad\textsc{+Yahoo}       &  $63.63$ & $71.84$ & $75.34$ & \quad\textsc{+Yahoo} & $\bm{\underline{54.33}}$ & $66.78$ &  $77.56$ & \quad\textsc{+DBPedia} & $30.13$ & $39.57$ & $51.39$ \\
\midrule
\textsc{MetricPrompt}     & $39.16$ & $65.77$ & $76.33$ & \textsc{MetricPrompt} & $32.31$ & $71.20$ & $88.44$ & \textsc{MetricPrompt} & $18.80$ & $28.76$ & $53.54$ \\
\quad\textsc{+DBPedia}     & $\underline{66.95}$ & $\underline{71.40}$ & $\underline{77.34}$ & \quad\textsc{+AG's News} & $\underline{53.23}$ & $\underline{74.21}$ & $\underline{88.34}$ & \quad\textsc{+AG's News} & $\underline{32.10}$ & $\bm{\underline{44.27}}$ & $\underline{52.29}$ \\
\quad\textsc{+Yahoo}       &  $\bm{\underline{71.00}}$ & $\bm{\underline{73.99}}$ & $\bm{\underline{79.57}}$ & \quad\textsc{+Yahoo} & $53.03$ & $\bm{\underline{76.41}}$ &  $\bm{\underline{89.47}}$ & \quad\textsc{+DBPedia} & $\bm{\underline{32.77}}$ & $\underline{43.63}$ & $\bm{\underline{53.78}}$ \\
\bottomrule
\end{tabular}
}
\centering
\caption{
The performance of MetricPrompt and ProtoVerb with additional OOD training data. 
Underlined number indicates the best result under the same setting. 
Bold number represents the best result on the dataset. 
}
\label{tbl: extensibility}
% \vspace{-5mm}
\vspace*{-3mm}
\end{table*}

Meanwhile, we have following observations based on Table~\ref{tbl: main_24} and Table~\ref{tbl: main_816}:

\textbf{(1)} MetricPrompt is the only and first prompting method outperforming ManualVerb without any human labor involved in task-specific verbalizer design. 
MetricPrompt benefits from paired input text, which introduces cross-sample information to make up the lack of the extra human knowledge and trial-and-error.
% We attribute MetricPrompt makes up the lack of the extra human knowledge by introducing cross-sample information to aid classification task. 
% It marks the first time when automatically designed verbalizer gains better performance than that of carefully hand-crafted ones. 

\textbf{(2)} MetricPrompt achieves the highest score over automatic verbalizer design methods. 
Compared with AVS, MetricPrompt does not restrict each class's representation to several sub-optimal words from the vocabulary, but instead represent it with corresponding training samples, leading to more accurate semantic representation. 
For the comparison with SoftVerb and ProtoVerb, we attribute MetricPrompt's leading performance to the smaller gap between its task formulation and PLM's pre-training objective. 
Unlike SoftVerb and ProtoVerb, MetricPrompt does not operate on PLM's inner representations, but functions with only the output word probability distribution at \texttt{[MASK]} position.
Moreover, MetricPrompt does not introduce task-specific parameters to be trained from scratch, avoiding over-fitting problem under few-shot scenarios. 

% \item MetricPrompt outperforms previous SOTA baselines by a smaller fraction as shot number increases.
% It indicates the marginal diminishing effect in few-shot learning: the larger the training set is, the less the semantic information introduced by extra samples. 
% As a result, models which cannot utilize few-shot samples as effectively as MetricPrompt still achieves comparable results as shot number increases. 

\textbf{(3)} MetricPrompt achieves comparable results with mean pooling and max pooling, but a performance drop is witnessed with KNN pooling.  
We ascribe the performance gap to the incompatibility between KNN pooling and the non-uniform distribution of MetricPrompt's predicted relevance scores.
% across training samples. 
We further discuss this phenomenon in Section~\ref{sec: 5_3}. 


% \begin{itemize}
%     \item MetricPrompt is the only and first prompting method outperforming ManualVerb without any human labor involved in task-specific verbalizer design. 
%     MetricPrompt benefits from paired input text, which introduces cross-sample information to make up the lack of the extra human knowledge and trial-and-error.
%     % We attribute MetricPrompt makes up the lack of the extra human knowledge by introducing cross-sample information to aid classification task. 
%     % It marks the first time when automatically designed verbalizer gains better performance than that of carefully hand-crafted ones. 
    
%     \item MetricPrompt achieves the highest score over automatic verbalizer design methods. 
%     Compared with AVS, MetricPrompt does not restrict each class's representation to several sub-optimal words from the vocabulary, but instead represent it with corresponding training samples, leading to more accurate semantic representation. 
%     For the comparison with SoftVerb and ProtoVerb, we attribute MetricPrompt's leading performance to the smaller gap between its task formulation and PLM's pre-training objective. 
%     Unlike SoftVerb and ProtoVerb, MetricPrompt does not operate on PLM's inner representations, but functions with only the output word probability distribution at \texttt{[MASK]} position.
%     Moreover, MetricPrompt does not introduce task-specific parameters to be trained from scratch, avoiding over-fitting problem under few-shot scenarios. 
    
%     % \item MetricPrompt outperforms previous SOTA baselines by a smaller fraction as shot number increases.
%     % It indicates the marginal diminishing effect in few-shot learning: the larger the training set is, the less the semantic information introduced by extra samples. 
%     % As a result, models which cannot utilize few-shot samples as effectively as MetricPrompt still achieves comparable results as shot number increases. 

%     \item MetricPrompt achieves comparable results with mean pooling and max pooling, but a performance drop is witnessed with KNN pooling.  
%     We ascribe the performance gap to the incompatibility between KNN pooling and the non-uniform distribution of MetricPrompt's predicted relevance scores.
%     % across training samples. 
%     We further discuss this phenomenon in Section~\ref{sec: 5_3}. 
    
% \end{itemize}

























==> 5_analysis.tex <==

\section{Analysis}
In this section, we further evaluate MetricPrompt from different aspects to illustrate its effectiveness. 


\subsection{Extensibility with Out-Of-Domain Data}
\label{sec: 5_1}
Although MetricPrompt performs well given sufficient training samples, its performance under 4 and fewer-shot settings far lags behind that trained with more labeled samples. 
In practice, however, we cannot always obtain enough labeled data in real world scenarios. 
Therefore, the proposed method's extensibility with Out-Of-Domain (OOD) data is crucial to its practicality. 
% its performance under four and fewer-shot settings far lags behind that trained with more labeled samples. 
% Therefore, the proposed method's extensibility with Out-Of-Domain (OOD) data is crucial to its practicality in real world scenarios where labeled data is usually sufficient. 

To demonstrate MetricPrompt's extensibility, we aid each dataset's few-shot classification with 16-shot training sets of other datasets. 
% To demonstrate MetricPrompt's extensibility, we introduce 16-shot training sets of DBPedia and Yahoo to aid AG's news dataset's classification.
We conduct experiments with 1, 2 and 4-shot settings, where the model's performance remains to be improved. 
We adopt mean pooling and simply mix up training samples of the original dataset and OOD ones to train the model. 
The inference process remains the same as that without OOD training data, where only training samples of the original dataset are involved. 
% For MetricPrompt, we adopt mean pooling and simply mix up training samples of the original dataset and OOD ones to train the model.  
For ProtoVerb baseline, we first train the model on OOD training data, and then re-initialize prototype parameters for the training on the original dataset. 

% As shown in Table~\ref{tbl: extensibility}, MetricPrompt still outperforms previous SOTA baseline ProtoVerb when boosted by OOD training data. 
As shown in Table~\ref{tbl: extensibility}, MetricPrompt achieves much higher accuracy when boosted by OOD training data. 
% The performance gap between fewer-shot and 16-shot settings are reduced by a large fraction. 
Compared with previous SOTA baseline ProtoVerb, MetricPrompt obtains better prediction accuracy in 17 out of 18 few-shot and OOD data settings (underlined numbers in the table). 
We can also observe that the fewer original training samples are, the more improvement OOD data brings about.
It can be explained by the marginal diminishing effect of extra training samples mentioned in Section~\ref{sec: 4_5}. 
Although OOD data improves the model's performance under most settings, AG's News training set fail to aid DBPedia 4-shot and Yahoo 4-shot performance.
We ascribe this failure to abundance of training samples under these settings. 
DBPedia and Yahoo contains 4096 and 1600 training samples under 4-shot setting, while AG's News 4-shot training set only contains 256 samples. 
As a result, the model is not trained sufficiently and can benefit from OOD data under AG's News 4-shot setting. 
For DBPedia and Yahoo, however, the model has adapted well to the relevance estimation task with in-domain data. 
OOD data serves more as noises and therefore harms the model's performance. 



% \begin{table}[t]
% \small
% \begin{tabular}{l c c c c c}
% \toprule
% Methods & 1-shot & 2-shot & 4-shot
% \\
% \midrule
% % ProtoVerb & $46.79$ & $58.38$ & $65.04$ \\
% % \quad+DBPedia & $57.62$ & $65.94$ & $71.19$ \\
% % \quad+Yahoo & $63.87$ & $71.99$ & $74.94$ \\
% \textsc{MetricPrompt} & $39.16$ & $65.77$ & $76.33$ \\
% \quad\textsc{+DBPedia} & $66.95$ & $71.40$ & $77.34$ \\
% \quad\textsc{+Yahoo} & $\bm{71.00}$ & $\bm{73.99}$ & $\bm{79.57}$ \\
% \bottomrule
% \end{tabular}
% \centering
% \caption{
% Model performance with OOD training data. 
% Bold numbers are the best results.
% }\label{tbl: extensibility}
% \end{table}

It is worth noticing that MetricPrompt's performance improvement under 1-shot setting is abnormally high. 
Without OOD data, MetricPrompt scores $39.16$, $32.31$, $18.80$ accuracy for the three datasets under 1-shot setting, underperforming ProtoVerb's $46.79$, $45.86$, $21.60$ accuracy. 
It is because MetricPrompt only takes two identical pieces of text as positive sample under 1-shot setting, leading to severe over-fitting problem. 
Consequently, the model does not analyze the semantic relevance information of the input text pair, but instead only produces high relevance score when given two identical text. 
The introduction of diversified OOD data alleviates the over-fitting problem effectively, and therefore improves MetricPrompt's 1-shot performance by a large fraction. 
MetricPrompt outperforms ProtoVerb in 5 out of 6 1-shot OOD data experiments, showing remarkable extensibility with OOD samples.


\subsection{Robustness against Noisy Samples}
Noisy samples harm model's performance in few-shot text classification tasks severely due to the lack of supervision signal. 
In this section, we evaluate MetricPrompt's robustness against noisy samples on AG's News dataset. 
Following~\citeauthor{cui2022prototypical}, we conduct experiments under 8 and 16-shot settings for training stability.
We replace 1, 2 and 4 training samples' labels randomly to introduce noises, and evaluate MetricPrompt's performance when equipped with mean, max and KNN pooling. 
We compare our method with previous SOTA baseline ProtoVerb, which shows the best robustness against noisy samples among automatic verbalizer design methods~\cite{cui2022prototypical}. 
The performance drop caused by noisy samples are displayed in Table~\ref{tbl: robustness}. 

\begin{table*}[t]
% \small
% \resizebox{\textwidth}{15mm}{
\begin{tabular}{l cc cc cc cc}
\toprule
\multicolumn{1}{c}{Method} &
\multicolumn{2}{c}{1 wrong} &
\multicolumn{2}{c}{2 wrong} &
\multicolumn{2}{c}{4 wrong} &
\multicolumn{2}{c}{Average}
\\
\cmidrule(lr{0.5em}){2-3}\cmidrule(lr{0.5em}){4-5}\cmidrule(lr{0.5em}){6-7}\cmidrule(lr{0.5em}){8-9}
& 8-shot & 16-shot & 8-shot & 16-shot & 8-shot & 16-shot & 8-shot & 16-shot \\
\midrule
\textsc{ProtoVerb}     & $2.79$ & $0.83$ & $4.95$ & $1.85$ & $11.31$ &  $3.71$ & $6.35$ & $2.13$ \\
\textsc{$\text{MetricPrompt}_{\text{knn}}$}     & $5.74$ & $2.61$ & $5.66$ & $3.08$ & $12.38$ &  $3.38$ & $7.93$ & $3.02$ \\
\textsc{$\text{MetricPrompt}_{\text{max}}$}     & $\bm{1.59}$ & $0.59$ & $3.12$ & $\bm{0.89}$ & $\bm{7.01}$ &  $\bm{1.21}$ & $3.91$ & $\bm{0.90}$ \\
\textsc{$\text{MetricPrompt}_{\text{mean}}$}     & $1.81$ & $\bm{0.55}$ & $\bm{2.72}$ & $1.04$ & $7.06$ & $1.52$ & $\bm{3.86}$ & $1.04$ \\
\bottomrule
\end{tabular}
% }
\centering
\caption{
Models' performance drop under AG's News 8 and 16-shot settings with 1, 2 and 4 noisy samples.
Bold number indicates the least drop among all methods.
}
\label{tbl: robustness}
% \vspace{-5mm}
\vspace*{-3mm}
\end{table*}

Compared with ProtoVerb, MetricPrompt suffers from less performance drop and achieves higher classification accuracy with mean and max pooling. 
Mean and max pooling obtain comparable results, but KNN pooling leads to much worse performance. 
KNN pooling suffers from a $7.93$ and $3.02$ accuracy drop under 8 and 16-shot setting, respectively. 
It is two times of the performance drop of mean pooling and max pooing. 
KNN pooling is the only pooling method performing worse than ProtoVerb. 
% Max pooling shows better robustness than mean pooling and KNN pooling, because max pooling only considers the highest relevance score, attenuating the influence of noisy samples. 
We attribute the large performance drop of KNN pooling to its incompatibility with the relevance score distribution of MetricPrompt and susceptibility to the variance of each class's training sample number.
We provide a detailed analysis in Section~\ref{sec: 5_3}.
% We measure the influence with the expected number of noisy samples involved in the computation of target class's relevance score.
% A detailed analysis in given in Section~\ref{sec: 5_3}.
% Noisy sample only harms the model's performance when it is predicted to be the most relevant one with the query sample. 
% Since incorrect knowledge about the noisy sample, which contradicts PLM's general knowledge, is injected to the model during training, it can hardly be regarded as the most relevant sample with the query one. 
% As a result, noisy samples only influence the model in few corner cases, leading to less performance drop. 
We can also observe that models' performance drops for a larger fraction under 8-shot setting than 16-shot one. 
Noisy signal takes up a larger part of 8-shot training set, and therefore influences MetricPrompt's prediction more severely and results into more performance drop. 
To summarize, the less training samples are, the more harm noisy samples do. 



\subsection{Comparison across Pooling Methods}
\label{sec: 5_3}
The choice of pooling method influences MetricPrompt's performance significantly. 
% and behaviors. 
In this section, we analyze different pooling methods with clean and noised training data to explain their performance gap. 

Firstly, we focus on clean data scenario without noisy samples.
We collect statistics of the distribution of relevance scores computed by MetricPrompt. 
We choose AG's News 2-shot setting and compute the average relevance score of each query sample's most relevant training sample, second most relevant training sample, etc. 
As shown in Fig~\ref{fig: 5_3_1}, the distribution of relevance scores is highly non-uniform. 
The highest relevance score is much larger than others, even larger than the sum of other scores.
The max relevance score therefore serves as a decisive factor in MetricPrompt with mean pooling, leading to similar behavior with max pooling. 
% Compared with the top two relevance scores, other scores distribute more evenly. 
% For KNN pooling, subtle difference in tail scores 
% Training samples of the correct label can slip into in the second half easily.
% Even if a correct sample gains the highest score, it cannot make up for wrongly distributed samples of the same class due to the voting strategy of KNN pooling.
% KNN pooling, however, adopts voting strategy, where the largest relevance score cannot determine the classification result, losing information 
KNN pooling, however, adopts voting strategy, where score value information is ignored and even the largest relevance score cannot determine the classification result.
Once other training samples of the correct label cannot achieve top $k$ relevance score, the classification result will be unpredictable. 
As a result, KNN pooling does not fit MetricPrompt's relevance score distribution and therefore makes more mistakes than other pooling methods do.

\begin{figure}[t]
\centering
\begin{tikzpicture}
\draw (0,0 ) node[inner sep=0] {\includegraphics[width=\columnwidth, trim={0cm 0cm 0cm -1cm}, clip]{./figs/distribution_blue.pdf}};
\end{tikzpicture}
\caption{
Average relevance scores between each query sample and all training samples under AG's News 2-shot setting. 
The scores are sorted and shifted to non-negative region.
}\label{fig: 5_3_1}
\end{figure}

\begin{figure*}[t]
\centering
\begin{tikzpicture}
\draw (0,0 ) node[inner sep=0] {\includegraphics[width=2\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{./figs/bias_blue_short.pdf}};
\end{tikzpicture}
\caption{
Average query sample number classified to classes with 7, 8 and 9 training samples under AG's News 8-shot setting. 
``\# Predicted query sample” indicates the average number of query samples predicted to the class. 
KNN pooling shows stronger preference to 9-sample classes than classes with fewer training samples. 
}\label{fig: 5_3_2}
\end{figure*}

We then analyze MetricPrompt's performance with noisy samples.
% Subtle difference in the evenly distributed tail relevance scores can 
% Noisy samples introduces variance into the number of training samples per class. 
As Fig~\ref{fig: 5_3_1} shows, the distribution of relevance scores except the top ones is relatively even. 
Supposing an extreme situation where the distribution of relevance scores is uniform, KNN pooling's prediction will be influenced by the variance of each class's training sample number significantly. 
Its voting mechanism regards each top $k$ most relevant training sample as one vote without taking relevance score value into consideration, and therefore develops a strong preference to classes with more training samples. 
On the contrary, mean pooling and max pooling considers each training sample's relevance score value information, so the influence of training sample number is mitigated. 
% by score value information. 
% Supposing an extreme situation where the distribution of relevance scores is uniform, the variance of each class's training sample number will influence KNN pooling's prediction significantly because of its voting mechanism.
% KNN pooling regards each top $k$ most relevant training sample as one vote, without taking relevance score value into consideration. 
Based on this observation, we argue that KNN pooling performs poorly when noisy samples are introduced because voting mechanism makes it susceptible to the variance of training sample number across classes. 
% To verify this, we collect statistics of the average predicted query sample number for classes with different training sample number and display the results in Table~\ref{tbl: 5_3}. 
To verify this, we first categorize classes of AG's News dataset 8-shot training sets according to the number of their corresponding training samples.
Then we collect statistics of the average predicted query sample number for each type of class. 
% Then we collect statistics of the average predicted query sample number for classes with different number of training samples. 
The statistics and standard deviation across classes with different number of training samples is shown in Fig~\ref{fig: 5_3_2} and Table~\ref{tbl: 5_3}.
% To verify this, we collect statistics of the average predicted query sample number for classes with different training sample number and report the standard deviation in Table~\ref{tbl: 5_3}. 
% The experiment is conducted under AG's News 8-shot setting.
% \begin{table}[t]
% \small
% \begin{tabular}{l c c c}
% \toprule
% Method & 0 wrong & 1 wrong & 4-shot
% \\
% \midrule
%  \textsc{Mean Pooling} & $44.05$ & $267.05$ & $254.33$ \\
%  \textsc{Max Pooling} & $246.13$ & $293.97$ & $275.34$ \\
%  \textsc{KNN Pooling} & $\bm{118.12}$ & $\bm{668.90}$ & $\bm{668.96}$ \\
% \bottomrule
% \end{tabular}
% \centering
% \caption{
% Standard deviation of predicted query sample number across classes with different training sample number.
% Bold numbers indicates the largest deviation.
% }\label{tbl: 5_3}
% \end{table}

% \begin{table}[t]
% \small
% \begin{tabular}{l c c c c c}
% \toprule
% Method & \#Noisy & 7-sample & 8-sample & 9-sample & std
% \\
% \midrule
% \multirow{2}{*}{\textsc{Mean Pooling}} & 1 & $1651$ & $1883$ & $2184$ & $267.05$ \\
%  & 4 & $1629$ & $1927$ & $2135$ & $254.33$ \\
% \midrule
% \multirow{2}{*}{\textsc{Max Pooling}} & 1 & $1643$ & $1865$ & $2226$ & $293.97$ \\
%  & 4 & $1607$ & $1929$ & $2154$ & $275.34$ \\
% \midrule
% \multirow{2}{*}{\textsc{KNN Pooling}} & 1 & $1209$ & $1923$ & $2546$ & $\bm{668.90}$ \\
%  & 4 & $1174$ & $1995$ & $2500$ & $\bm{668.96}$ \\
% \bottomrule
% \end{tabular}
% \centering
% \caption{
% Average query sample number classified to classes with 7, 8 and 9 training samples under AG's News 8-shot setting. 
% ``\#Noisy” indicates the number of noisy samples in the training set. 
% ``std” refers to query sample number standard deviation across classes with different number of training samples. 
% % Standard deviation of predicted query sample number across classes with different training sample number. 
% Bold numbers indicates the largest deviation in the noisy sample setting.
% }\label{tbl: 5_3}
% \end{table}

As we can observe in Fig~\ref{fig: 5_3_2}, KNN pooling shows significantly stronger preference to classes with more training samples than mean pooling and max pooling do.
When one noisy sample is introduced to the training set, mean pooling classifies 533 more query samples to classes with 9 training samples than those with 7 training samples averagely. 
On the contrary, KNN pooling classifies 1337 more query samples to 9-sample classes than 7-sample classes, which is 1.5 times larger than that of mean pooling. 
The standard deviation statistics shown in Table~\ref{tbl: 5_3} indicates the same tendency.
KNN pooling's predicted query sample number across classes is highly inconsistent, resulting into a 668.90 predicted query sample number standard deviation when one noisy sample is introduced. 
The standard deviation of mean pooling is 267.05 under the same setting for comparison. 
% The predicted query sample number standard deviation of mean pooling is 267.05 under the same setting for comparison. 
% KNN pooling strong preference to certain classes and abnormally high predicted query sample number deviation 
KNN pooling's voting strategy ignores score value information, and even the highest relevance score is only counted as one vote.
Since the distribution of MetricPrompt's relevance score except the top ones is relatively even, KNN pooling develops strong preference to certain classes and abnormally high predicted query sample number deviation. 
% Given the even distribution of MetricPrompt's relevance score, KNN pooling develops strong preference to certain classes and abnormally high predicted query sample number deviation. 
As indicated by the statistics, KNN pooling classifies a large number of query samples to classes with more training samples, including those belonging to other classes. 
Therefore, a large drop in KNN pooling's performance is witnessed when noisy samples are introduced to the training set.

% The variance in training sample number across classes increase the standard deviation of each method's predicted query sample number across classes.
% The deviation increase of KNN pooling is abnormally high, indicating its strong dependence to training sample number distribution. 
% KNN pooling is severely biased to classes with more training samples. 
% Averagely for four noisy samples setting, we observe KNN pooling to classify 2500 query samples to classes with 9 training samples, while only 1174 are classified to those with only 7 training samples.
% The corresponding statistics for mean pooling is 2135 and 1629.
% % bias to classes with more training samples. 
% % Because the variance in training set size is introduced by noisy samples, performance of KNN pooling drops the most among all pooling methods.
% KNN pooling's voting strategy loses score value information, and is therefore susceptibility to the distribution of training sample numbers, resulting into worse performance with noisy samples.

\begin{table}[t]
\small
\begin{tabular}{c c c c}
\toprule
\# Noisy sample & \textsc{Mean Pooling} & \textsc{Max Pooling} & \textsc{KNN Pooling}
\\
\midrule
 1 & $267.05$ & $293.97$ & $\bm{668.90}$ \\
 4 & $254.33$ & $275.34$ & $\bm{668.96}$ \\
\bottomrule
\end{tabular}
\centering
\caption{
Standard deviation of predicted query sample number across classes with different training sample number. 
``\# Noisy sample” refers to the number of noisy samples. 
Bold number indicates the largest deviation.
}\label{tbl: 5_3}
\end{table}


\subsection{Influence of Pivot Sample Number}
Although MetricPrompt achieves promising text classification accuracy, the time-consuming inference process may limit its applicability in real world text classification scenarios with high demands on execution speed. 
We propose to use pivot samples to reduce the time complexity of the inference stage to be the same with other prompting methods. 
In this part, we investigate the influence of pivot sample number per class to the performance of MetricPrompt. 
We conduct experiments on the three datasets across four few-shot settings with pivot sample number $p$ set as 1, 2 and 4. 
We display the average performance under different few-shot settings in Table~\ref{tbl: 5_4}. 
Complete experiment results are shown in Appendix~\ref{}. 

As shown in Table~\ref{tbl: 5_4}, the performance of MetricPrompt positively correlate with the number of pivot samples. 
As the number of pivot samples increase, MetricPrompt captures each label's semantic meaning more accurately and therefore achieves better performance. 
It is worth noticing that even if only one pivot sample is selected for each class, MetricPrompt still outperforms ProtoVerb's $49.36$, $60.85$, $71.96$, $79.68$ classification accuracy under the four few-shot settings. 
The selection of pivot sample number $p$ serves as a trade-off between classification accuracy and efficiency.
In real world applications, MetricPrompt can adapt to varying scenarios with different requirements by adjusting the number of pivot samples. 
% hen applied in real world text classification scenarios


\begin{table}[t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{l c c c c}
\toprule
Method & 2-shot & 4-shot & 8-shot & 16-shot
\\
\midrule
 \textsc{ProtoVerb} & $49.36$ & $60.85$ & $71.96$ & $79.68$ \\
 \textsc{$\text{MetricPrompt}_{1\text{pivot}}$}  & $50.90$ & $67.97$ & $76.60$ & $80.45$ \\
 \textsc{$\text{MetricPrompt}_{2\text{pivot}}$}  & $\bm{55.24}$ & $70.66$ & $77.98$ & $80.72$ \\
 \textsc{$\text{MetricPrompt}_{4\text{pivot}}$}  & $\bm{55.24}$ & $\bm{72.77}$ & $\bm{78.25}$ & $\bm{81.01}$ \\
\bottomrule
\end{tabular}
}
\centering
\caption{
The performance of MetricPrompt with different number of pivot samples.
Each result in the table is the average performance across the three datasets. 
``\# Pivot sample” refers to the number of pivot samples per class. 
Bold number indicates the largest deviation.
}\label{tbl: 5_4}
\end{table}







































































































